Subset Feedback Vertex Set in Chordal and Split Graphs

In the \textsc{Subset Feedback Vertex Set (Subset-FVS)} problem the input is a graph $G$, a subset \(T\) of vertices of \(G\) called the `terminal' vertices, and an integer $k$. The task is to determine whether there exists a subset of vertices of cardinality at most $k$ which together intersect all cycles which pass through the terminals. \textsc{Subset-FVS} generalizes several well studied problems including \textsc{Feedback Vertex Set} and \textsc{Multiway Cut}. This problem is known to be \NP-Complete even in split graphs. Cygan et al. proved that \textsc{Subset-FVS} is fixed parameter tractable (\FPT) in general graphs when parameterized by $k$ [SIAM J. Discrete Math (2013)]. In split graphs a simple observation reduces the problem to an equivalent instance of the $3$-\textsc{Hitting Set} problem with same solution size. This directly implies, for \textsc{Subset-FVS} \emph{restricted to split graphs}, (i) an \FPT algorithm which solves the problem in $\OhStar(2.076^k)$ time \footnote{The \(\OhStar()\) notation hides polynomial factors.}% for \textsc{Subset-FVS} in Chordal % Graphs [Wahlstr\"om, Ph.D. Thesis], and (ii) a kernel of size $\mathcal{O}(k^3)$. We improve both these results for \textsc{Subset-FVS} on split graphs; we derive (i) a kernel of size $\mathcal{O}(k^2)$ which is the best possible unless $\NP \subseteq \coNP/{\sf poly}$, and (ii) an algorithm which solves the problem in time $\mathcal{O}^*(2^k)$. Our algorithm, in fact, solves \textsc{Subset-FVS} on the more general class of \emph{chordal graphs}, also in $\mathcal{O}^*(2^k)$ time.

==> preamble.tex <==
\makeatletter
% define a macro \Autoref to allow multiple references to be passed to \autoref
\newcommand\Autoref[1]{\@first@ref#1,@}
\def\@throw@dot#1.#2@{#1}% discard everything after the dot
\def\@set@refname#1{%    % set \@refname to autoefname+s using \getrefbykeydefault
    \edef\@tmp{\getrefbykeydefault{#1}{anchor}{}}%
    \xdef\@tmp{\expandafter\@throw@dot\@tmp.@}%
    \ltx@IfUndefined{\@tmp autorefnameplural}%
         {\def\@refname{\@nameuse{\@tmp autorefname}s}}%
         {\def\@refname{\@nameuse{\@tmp autorefnameplural}}}%
}
\def\@first@ref#1,#2{%
  \ifx#2@\autoref{#1}\let\@nextref\@gobble% only one ref, revert to normal \autoref
  \else%
    \@set@refname{#1}%  set \@refname to autoref name
    \@refname~\ref{#1}% add autoefname and first reference
    \let\@nextref\@next@ref% push processing to \@next@ref
  \fi%
  \@nextref#2%
}
\def\@next@ref#1,#2{%
   \ifx#2@ and~\ref{#1}\let\@nextref\@gobble% at end: print and+\ref and stop
   \else, \ref{#1}% print  ,+\ref and continue
   \fi%
   \@nextref#2%
}

\makeatother


\usepackage{charter}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage{amsfonts}
%\usepackage{amsthm}
%\usepackage{amsthm,cleveref} % For getting autoref names correct with
                      % shared counters. Also, this combination infers environment names.
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{thmtools,thm-restate}
%\declaretheorem{theorem}
%\usepackage{fullpage}
\usepackage{enumitem}
%\usepackage{subcaption} % For figures inside figures
% The above has issues with the llncs class.
\usepackage[caption=false]{subfig}

\usepackage{microtype}%if unwanted, comment out or use option "draft"
\usepackage{complexity}
\usepackage{todonotes}
\usepackage[utf8]{inputenc}
\usepackage{xspace}
\usepackage{float}
\usepackage{graphicx}
\usepackage{capt-of}% or \usepackage{caption}
\usepackage{booktabs}
\usepackage{varwidth}
\usepackage{textcomp} % For drawing double-hyphens.

% Extended Abstract
\usepackage{pdfpages}

% Draft
\newcommand{\remove}[1]{}
\newcommand{\discuss}[1]{\textcolor{CadetBlue}{[#1]}}

 
\newcommand{\name}[1]{\textsc{#1}}

% Problems 
\newcommand{\dHS}{\name{$d$-Hitting Set}\xspace}
\newcommand{\VC}{\name{Vertex Cover}\xspace}
\newcommand{\PC}{\name{Point Covering}\xspace}
\newcommand{\PLC}{\name{Point Line Cover}\xspace}
\newcommand{\LPC}{\name{Line Point Cover}\xspace}
\newcommand{\TSP}{\name{Travelling Salesperson Problem}\xspace}
\newcommand{\MBTSP}{\name{Minimum Bends Travelling Salesperson Problem}\xspace}

% Complexity classes
%\newcommand{\NPH}{$\mathsf{NP}$-hard\xspace}
%\newcommand{\FPT}{\ensuremath{\mathsf{FPT}}\xspace}
%\newcommand{\APXH}{$\mathsf{APX}$-hard\xspace}
%\newcommand{\conjecture}{\ensuremath{\mathsf{coNP} \nsubseteq \mathsf{NP/poly}}\xspace}
\newcommand{\caveat}{\ensuremath{\mathsf{coNP} \subseteq \mathsf{NP/poly}}\xspace}

% Sets

% For problem definitions
\newcommand{\defparproblem}[4]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3
\\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{1mm}
}
% \newenvironment{decnamedefn}[3]{
% \par\addvspace{0.4\baselineskip}\fbox{%
% \begin{minipage}[t]{0.95\textwidth}%
% \begin{tabular}{p{0.15\textwidth}p{0.80\textwidth}}
%     \multicolumn{2}{l}{\name{#1}} \\
%         \textsl{Input:} & {#2} \\ %\hspace{1.2cm} \= \parbox[t]{10.7cm}{#2} \\
%         \textsl{Question:} & {#3} \\%            \> \parbox[t]{10.7cm}{#3} 
%    \end{tabular}
% \end{minipage}}\par\addvspace{0.4\baselineskip}
% }
\newenvironment{decnamedefn}[3]{
\par\medskip\noindent\fbox{%
\begin{minipage}[t]{0.985\textwidth}%
\begin{tabular}{p{0.15\textwidth}p{0.80\textwidth}}
    \multicolumn{2}{l}{\name{#1}} \\
        \textsl{Input:} & {#2} \\ %\hspace{1.2cm} \= \parbox[t]{10.7cm}{#2} \\
        \textsl{Question:} & {#3} \\%            \> \parbox[t]{10.7cm}{#3} 
   \end{tabular}
\end{minipage}}\par\addvspace{0.4\baselineskip}
}

% \newenvironment{parnamedefn}[4]{
% \par\addvspace{0.4\baselineskip}\fbox{%
% \begin{minipage}[t]{0.95\textwidth}%
% \begin{tabular}{p{0.15\textwidth}p{0.80\textwidth}}
%     \multicolumn{2}{l}{\name{#1}} \\
%         \textsl{Input:} & {#2} \\ %\hspace{1.2cm} \= \parbox[t]{10.7cm}{#2} \\
%         \textsl{Question:} & {#3} \\%            \> \parbox[t]{10.7cm}{#3} 
%         \textsl{Parameter:} & {#4} \\%
%    \end{tabular}
% \end{minipage}}\par\addvspace{0.4\baselineskip}
% }
\newenvironment{parnamedefn}[4]{
\par\medskip\noindent\fbox{%
\begin{minipage}[t]{0.985\textwidth}%
\begin{tabular}{p{0.14\textwidth}p{0.80\textwidth}}
    \multicolumn{2}{l}{\name{#1}} \\
        \textsl{Input:} & {#2} \\ %\hspace{1.2cm} \= \parbox[t]{10.7cm}{#2} \\
        \textsl{Question:} & {#3} \\%            \> \parbox[t]{10.7cm}{#3} 
        \textsl{Parameter:} & {#4} \\%
   \end{tabular}
\end{minipage}}\par\addvspace{0.4\baselineskip}
}

% Theorem-like environments
%\theoremstyle{plain} % Theorems, lemmas, propositions
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{fact}{Fact}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newcommand{\conjectureautorefname}{Conjecture}
%\newtheorem{observation}{Observation}[section]
%\newcommand{\observationautorefname}{Observation}
%\newtheorem{proposition}{Proposition}[section]
%\newcommand{\propositionautorefname}{Proposition}
%\newtheorem{corollary}{Corollary}[section]
%\newcommand{\corollaryautorefname}{Corollary}
%\newtheorem{lemma}{Lemma}[section]
%\newcommand{\lemmaautorefname}{Lemma}

% ... for llncs.cls
\spnewtheorem{fact}{Fact}{\bfseries}{\itshape}
%\newcommand{\factautorefname}{Fact}
\spnewtheorem{observation}{Observation}{\bfseries}{\itshape}
%\newcommand{\observationautorefname}{Observation}
\spnewtheorem{reductionrule}{Reduction~Rule}{\bfseries}{\itshape}
%\newcommand{\reductionruleautorefname}{Reduction~Rule}
\spnewtheorem{branchingrule}{Branching~Rule}{\bfseries}{\itshape}
%\newcommand{\branchingruleautorefname}{Branching~Rule}
%% llncs.cls defines a stupid claim environment with no numbering.
\spnewtheorem{claimnr}{Claim}{\bfseries}{\itshape} 
%\newcommand{\claimnrautorefname}{Claim}


%\theoremstyle{remark} % Remarks, notes
%\newtheorem{remark}{Remark}[section] 
%\newcommand{\remarkautorefname}{Remark}
%\newtheorem{reductionrule}{Reduction~Rule}[section]
%\newcommand{\reductionruleautorefname}{Reduction~Rule}
%\newtheorem{branchingrule}{Branching~Rule}[section]
%\newcommand{\branchingruleautorefname}{Branching~Rule}

%\theoremstyle{definition} % For definitions
%\newtheorem{definition}{Definition}[section]
%\newcommand{\definitionautorefname}{Definition}
\newcommand{\sectionautorefname}{Section}

\newcommand{\NO}{\textsf{NO}\xspace}
\newcommand{\YES}{\textsf{YES}\xspace}
\newcommand{\Oh}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\OhStar}{\ensuremath{\mathcal{O}^{\star}}\xspace}


\newcommand{\SubsetFVSChordal}{\textsc{Subset FVS in Chordal Graphs}\xspace}
\newcommand{\SFVSC}{\textsc{Subset FVS in Chordal Graphs}\xspace} % shorter version
\newcommand{\SubsetFVSSplit}{\textsc{Subset FVS in Split Graphs}\xspace}
\newcommand{\SFVSS}{\textsc{Subset FVS in Split Graphs}\xspace} % shorter version

% Commands from here till \begin{document} were added by Varun
\newcommand{\oh}[1]{\mathcal{O}$($#1$)$}
\newcommand{\yes}{\textsf{YES}\xspace}
\newcommand{\no}{\textsf{NO}\xspace}

\newcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\dunion}{\mathbin{\mathaccent\cdot\cup}}
\renewcommand{\emptyset}{\text{\O}}
\usepackage{enumitem}

\setcounter{tocdepth}{4}

\usepackage{xcolor}
\definecolor{linkcolor}{RGB}{170,0,0} % aa0000
\definecolor{citecolor}{RGB}{44,160,46} % 2ca02d
\definecolor{urlcolor}{RGB}{0,51,153} % 003399
\usepackage[]{hyperref}
\hypersetup{%
  pdftex,%
  pdfpagelabels,%
  bookmarks,%
  hyperindex,%
  hyperfigures,%
  linktocpage,%
  colorlinks=True,%
  urlcolor=urlcolor,%
  citecolor=citecolor,%
  linkcolor=linkcolor,%
  bookmarksnumbered=True,%     
  bookmarksopen=True,%         
  bookmarksopenlevel=1,%       
  pdfpagemode=UseOutlines,%
  hidelinks=True% THIS OPTION takes away link colours, while still
                % keeping them clickable. 
  }


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "subsetFVS"
%%% End: 

